Estimating Egocentric 3D Human Pose in Global Space

Egocentric 3D human pose estimation using a single fisheye camera has become popular recently as it allows capturing a wide range of daily activities in unconstrained environments, which is difficult for traditional outside-in motion capture with external cameras. However, existing methods have several limitations. A prominent problem is that the estimated poses lie in the local coordinate system of the fisheye camera, rather than in the world coordinate system, which is restrictive for many applications. Furthermore, these methods suffer from limited accuracy and temporal instability due to ambiguities caused by the monocular setup and the severe occlusion in a strongly distorted egocentric perspective. To tackle these limitations, we present a new method for egocentric global 3D body pose estimation using a single head-mounted fisheye camera. To achieve accurate and temporally stable global poses, a spatio-temporal optimization is performed over a sequence of frames by minimizing heatmap reprojection errors and enforcing local and global body motion priors learned from a mocap dataset. Experimental results show that our approach outperforms state-of-the-art methods both quantitatively and qualitatively.

==> Sections/introduction_old.tex <==
\section{Introduction}
% With a single downward looking fisheye camera, our goal is to estimate a person’s pose sequence for a variety of complex motions.


% Egocentric 3D human pose estimation is an important problem. 
%Traditional optical human motion capture techniques employ externally placed cameras that observe the human in an outside-in view. 
Traditional optical motion capture system with external, outside-in facing cameras is extremely restrictive for many pose estimation applications that require the person to be able to roam around in a larger space, beyond a fixed recording volume. Examples are mobile interaction applications, pose estimation in large-scale workplace environments, or many AR/VR applications.
%With the high demand for capturing 3D human poses in an unconstrained environment, 
To enable this, methods for egocentric 3D human pose estimation using
% [WXU: let's be a bit more general here] 
% a single mobile camera (head- or body-mounted)
head- or body-mounted cameras were researched.
%Unlike traditional setups for 3D human pose estimation (e.g. a single or multiple cameras placed statically around the subject), 
These methods are mobile, flexible, and have the potential to capture a wide range of daily human activities even in large-scale cluttered environments.
%(e.g. cameras need to be close to the subject, no occluders in front of the subject, etc), 
%which makes capturing a wide range of human activities in daily life possible 
% for example for action recognition, performance analysis~\cite{DBLP:journals/tvcg/XuCZRFST19} and $x$R (including VR, AR and MR) applications~\cite{DBLP:conf/iccv/TomePAB19}. 

\begin{figure}
	\begin{center}
		\includegraphics[width=0.97\linewidth]{Figures/ioexample/io-cap-3-crop.pdf}
	\end{center}
	\caption{Given challenging egocentric videos, our method produces realistic and accurate 3D global pose sequence.}
	\label{fig:io}
\end{figure}

%Limitations of existing works
Some egocentric capture methods study the estimation of face~\cite{Elgharib2020egocentricconferencing, elgharib2019egoface, DBLP:journals/tog/LiTOWTHNM15} and hand motions~\cite{Singh2016ActionRecon, SridharFastHandTracker, DBLP:conf/cvpr/MaFK16, DBLP:journals/pr/SinghAJ17}, while the estimation of the global full body pose has been less explored.  Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} and $x$R-egopose~\cite{DBLP:conf/iccv/TomePAB19} use a single non-facing head-mounted fisheye camera to capture the 3D skeletal body pose in a marker-less way. 
%the view of full body and estimate 3D body pose with respect to the fisheye camera. 
Both methods have demonstrated compelling 3D pose estimation results, but still have several limitations: (i) Both approaches estimate the local 3D body pose in egocentric camera space, rather than global rotation and translation in the 3D world coordinate system. Henceforth, we will refer to the former as ``local pose", in order to distinguish it from the ``global pose"  defined in the world coordinate system. Local pose capture alone is insufficient for many applications. For example, captured local body poses are not enough to animate the locomotion of a virtual avatar in $x$R environments, which requires global poses. 
% \CT{the following sentence may be not such a strong argument, maybe remove} Egocentric local pose capture can also cause ambiguities during action recognition; e.g, when disambiguating motions caused by turning the head or the entire body, for example.
% Obtaining the global translation and rotation of the body is difficult. One possible method is to simultaneously record the sequence with a multi-view setup. However,this would totally lose the advantages of using the mobile equipment. An alternative is to ... 
(ii) The estimated poses often exhibit notable temporal jitter, because video frames are processed independently without taking frame coherence into consideration. (iii) In the strongly distorted head-mounted fisheye perspective, the body is more often self-occluded, which may cause tracking failures. Also, capturing the lower body from the fisheye view is typically less stable, as it is much smaller in the camera view.  
%features mre freyqnet body self-occlusions than exocentric perpsectives perspective distortions and self-occlusions in the captured video lead to erroneous pose estimation. 



%Introduce our method
To tackle these challenges, we propose a novel method for egocentric global 3D human body pose estimation using a single head-mounted fisheye camera, as illustrated in Fig.~\ref{fig:io}. 
%Our approach 
%utilizes neural network-based local pose inference, whose reuslts are refined with the use of learned motion priors and a combinaton of egocentric SLAM and space-time optimization-based global pose refinement.
%In order to obtain accurate and temporally stable global poses, we incorporate body motion priors learned from the large mocap dataset of AMASS~\cite{AMASS:ICCV:2019} into a two-stage optimization for local pose and global pose separately. In this process, to alleviate the influence of the perspective distortion and self-occlusions in the captured video, we define a new uncertainty-aware reprojection loss for local pose optimization. 
Input to our approach is 
%an egocentric fisheye video sequence from a head-mounted camera. 
an egocentric video sequence from a head-mounted fisheye camera.
First, we compute the local 3D pose and 2D joint heatmap of each frame using a CNN-based local pose estimation method, and estimate 3D transformation between subsequent frames using a SLAM approach~\cite{murTRO2015}. 
% We note that our method can work with any local pose estimation method. In most of our experiments, we use  Mo2cap2~\cite{DBLP:journals/tvcg/XuCZRFST19}, but we also evaluate our approach with the results of xR-egopose~\cite{DBLP:conf/iccv/TomePAB19} as inputs.
Subsequently, a spatio-temporal optimization is performed that computes a refined, more accurate and temporally more stable sequence of local and global poses. To this end, in order to mitigate the ambiguities caused by strong self-occlusion, we designed an energy function that encodes the local and global pose prior, each of which is represented as variational autoencoder (VAE) trained on the AMASS dataset~\cite{AMASS:ICCV:2019}.
The energy function is minimized over a sequence of frames that measures 3D pose reprojection accuracy into 2D joint detections while enforcing similarity to the initial local pose and global camera estimates in a spatio-temporal way. 
% Considering the ambiguities caused by 
%strongly distorted fisheye perspective, 
% the strong self-occlusion,
%we calculate the reprojection loss term by accumulating the probability values at the heatmap pixels where the 3D estimated joints projected rather than comparing the projection of 3D estimated joints against 2D joint prediction. 
To further leverage the uncertainty captured in the heatmap, we calculate the reprojection loss term by summing up the probability values at the pixels on the heatmap occupied by the projection of the 3D estimated joints rather than comparing the projection of 3D estimated joints against 2D joint predictions. 
% \LJ{2D joint prediction -> `the 2D joint prediction estimated from the heatmap'?}.
% \CT{following sentence unclear - revise} To better handle distortion and self-occlusion in the captured video, instead of comparing the projection of 3D estimated joints against 2D joint prediction, we define a new uncertainty-aware reprojection loss by accumulating the probability values at the pixels on the heatmap that the 3D estimated joints projected. 
% Our optimization approach also enforces similarity to a local and global motion prior, each of which represented as variational autoencoder (VAE) trained on the AMASS dataset~\cite{AMASS:ICCV:2019}. The motion priors help to reduce the depth ambiguity and the uncertainty of the detection due to occlusions.


%To make the local pose more temporally stable and more accurate, we train a sequential variational autoencoder (VAE) on the AMASS dataset~\cite{AMASS:ICCV:2019} to encode local motion prior for local pose optimization. 
%Considering the ambiguity caused by the distortion and self-occlusion in the captured video, instead of comparing the projection of 3D estimated joints against 2D joint prediction, we define a new uncertainty-aware reprojection loss by accumulating the probability values at the pixels on the heatmap that the 3D estimated joints projected. 
%Next, the optimized local poses are converted into initial global poses with the estimated camera motion. In order to make the initial global poses more realistic, we impose the constraint that the optimized local body poses be in accordance with the corresponding camera poses. This is achieved by using a second VAE to learn global pose prior from the AMASS dataset~\cite{AMASS:ICCV:2019} for global pose optimization. 

We evaluate our method on the dataset provided by Mo$^2$Cap$^2$~\cite{DBLP:journals/tvcg/XuCZRFST19} and also a new benchmark dataset we collected with 2 subjects performing various motions. Our method outperforms the state-of-the-art methods both quantitatively and qualitatively. Our ablative analysis confirms the efficacy of our proposed optimization algorithm with learned motion prior and uncertainty aware reprojection loss for improved local and global accuracy and temporal stability.  
% \WX{Say something stronger to emphasize the vae pose prior.
% For instance, the motion priors help to reduce the depth ambiguity and the uncertainty of the detection due to occlusions.
% }
%Our extensive ablation studies demonstrate that incorporating motion priors into egocentric body pose estimation efficiently improves both the local pose and global pose in terms of accuracy and temporal stability, and that our new uncertainty-aware reprojection loss further increases the accuracy of local pose estimation so leads to better global pose estimation. 

In summary, our technical contributions are:
\begin{itemize}
    \item A novel approach for global 3D human pose estimation from an egocentric fisheye camera.
    \item A combination of CNN-based local pose and optimization-based global pose estimation with the assistance of separate local and global motion priors.
    \item A new uncertainty-aware reprojection loss to alleviate the adverse influence of the perspective distortion and self-occlusions in the captured video.
\end{itemize}




% In this paper, in order to tackle the aforementioned issues, we present a 2-step optimization framework that incorporates learned motion prior to obtain the realistic global 3D pose from egocentric video (See Fig.~\ref{fig:io}).
% %The pose sequences predicted by network are firstly optimized by a VAE-based local pose optimizer, then transformed into global space and finally optimized by the VAE-based global pose optimizer. 
% Our optimization framework can be simply attached to available egocentric pose estimation pipelines (including methods in \cite{DBLP:journals/tvcg/XuCZRFST19} and \cite{DBLP:conf/iccv/TomePAB19}) and efficient for real-time applications (50 frame/s).

% In order to exploit the temporal consistency and further make the predicted sequences more realistic, we leverage the motion prior to optimize the local pose sequence. In order to capture the motion prior, we train a sequential variational autoencoder (VAE) on a large-scale 3D motion-capture dataset called AMASS \cite{AMASS:ICCV:2019}. By incorporating this VAE, we can eliminate pose jittering and improve the prediction accuracy.

% To tackle the second challenging issue, we propose a new energy term in the local pose optimizer by considering the uncertainty in 2D joint estimations. We calculate the reprojection loss by accumulating heatmap values on reprojected 2D points rather than comparing them with 2D predictions. By using the heatmap-based reprojection energy, we are able to reduce the influence of inaccurate 2D predictions and ambiguous egocentric frames.

% To finally obtain the global 3D pose rather than the local pose, a straightforward solution is to transform the local pose by using the camera pose estimations from the SLAM. One prior is that the global camera pose must keep in accordance with the local body pose to make the resulting global body motion look realistic. To guarantee this, we introduce a second VAE-based global pose optimization block to regularize the obtained global pose. This optimizer is initialized with the local pose sequence from the local pose optimizer %and the camera pose sequence from the SLAM,%
% and finally gives the regularized pose in the global space.

% Besides, we have evaluated our method under real datasets collected by Xu et al. \cite{DBLP:journals/tvcg/XuCZRFST19} and us. Our method outperforms previous methods \cite{DBLP:journals/tvcg/XuCZRFST19, DBLP:conf/iccv/TomePAB19} with higher accuracy and more reasonable global body predictions.

% In summary, our contribution can be distributed into three aspects. Firstly, we have developed a fast motion prior based optimization approach for optimizing the pose sequence. Secondly, we have introduced the heat map reprojection loss rather than the normal reprojection loss for leveraging the uncertainty in the predicted heatmap. Finally, by using the SLAM and VAE based global regularizer, we further mitigate the ambiguity in pose estimation and get the accurate and reasonable global 3D pose sequence.



% Most of available works only focus on the estimation of body part motions, such as the facial expressions \cite{Elgharib2020egocentricconferencing, elgharib2019egoface, DBLP:journals/tog/LiTOWTHNM15} and hand activities \cite{Singh2016ActionRecon, SridharFastHandTracker, DBLP:conf/cvpr/MaFK16, DBLP:journals/pr/SinghAJ17}, while the estimation of whole-body pose is seldom explored. 


% Some recent works \cite{DBLP:conf/cvpr/JiangG17a, yuan20183d, DBLP:conf/iccv/YuanK19} infers 3D body pose from the implicit clues in the egocentric video stream. However, the predicted pose lacks accuracy because the human body is out of the camera's field of view. 
 

% Xu et al. \cite{DBLP:journals/tvcg/XuCZRFST19} and Tome et al. \cite{DBLP:conf/iccv/TomePAB19} introduce the head-mounted fisheye camera to capture the view of the whole body, thus enabling the estimation of 3D body pose from a single egocentric camera. However, these approaches suffer from three issues:  1. These approaches estimate the body pose frame-by-frame without exploiting the temporal consistency over a consecutive sequence, making the estimated pose sequence unlikely to appear in the real world. 2. the extreme perspective effects and self-occlusions under the egocentric camera viewpoint leads to strong ambiguity and further reduces the accuracy of the estimated pose. 3. These methods only estimates 3D joint positions relative to the head-mounted fisheye camera (local pose) and not able to obtain the 3D pose under the global coordinate system (global pose).



